Truthful Self-Play

We present a general framework for evolutionary learning to emergent unbiased state representation without any supervision. Evolutionary frameworks such as self-play converge to bad local optima in case of multi-agent reinforcement learning in non-cooperative partially observable environments with communication due to information asymmetry. Our proposed framework is a simple modification of self-play inspired by mechanism design, also known as {\em reverse game theory}, to elicit truthful signals and make the agents cooperative. The key idea is to add imaginary rewards using the peer prediction method, i.e., a mechanism for evaluating the validity of information exchanged between agents in a decentralized environment. Numerical experiments with predator prey, traffic junction and StarCraft tasks demonstrate that the state-of-the-art performance of our framework.

==> concepts/bengios-statement.tex <==
%Bengio \citep{bengio} describes the relationship between symbols and neural nets as follows:
\begin{quote} 
{\em ``\dots a human brain can learn such high-level abstractions if guided by
the messages produced by other humans, which act as hints or indirect supervision for these
high-level abstractions; and, language and the recombination and optimization of mental
concepts provide an efficient evolutionary recombination operator,  
and this gives rise to rapid search in the space of communicable ideas that help humans build up better high-level internal representations of their world.''} \citep{bengio}
\end{quote} 


==> concepts/psrs.tex <==
\begin{table*}[!t]
\centering
\caption{Examples of the proper scoring rules, where $\kappa> 1,\| p\|_\kappa=(\int p (a)^\kappa \dd a)^{1/\kappa} $. Readers can refer to \citep{psr} for other examples. }
\label{tbl:scoring}
\begin{tabular}{llccc}
\hline
& $\hspace{1.8em}\Action $ 
& $\Message $ 
& $\psi (p) $ 
& $\ell_{\psi}(a|z) $\\\hline
Logarithmic 
& Discrete 
& C
& $\Ent{p} $ 
& $\log\policy (a | z) $\\
Zero-one 
& Discrete 
& D
& $p $ 
& $\policy (a | z) $\\
Quadratic \small{\citep{brier1950verification} }
& Continuous 
& D
& $-\| p\|^2_2 $ 
& $ -2\policy (a | z)+\|\policy (\cdot | z)\|^2_2 $\\
Pseudospherical \small{\citep{good1992rational} }
& Continuous 
& C
& $-\| p\|^{\kappa-1}_\kappa $ 
& $-\policy (a | z)^{\kappa-1}/{\|\policy (\cdot | z)^\kappa\|^{\kappa-1}_\kappa} $\\\hline
\end{tabular}
\end{table*}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> problem/local-optimally.tex <==

Hence, maximizing the welfare is as same as {\em unbiased} optimization in self-play. 
We define the best welfare $\hat{J}(\Gn):= \sup_{\vect{w}} J(\vect{w}; \Gn)$ and diminished welfare at the equilibrium $J^*(\Gn):=J(\vect{w}^*; \Gn) $. By definition, $\hat{J}\ge J^* $ always holds.

\begin{prp} (global optimally)
    If $ \Gn \in \GameSpace $ is strongly truthful, $ J^*(\Gn) = \hat{J}(\Gn) $ holds and $\Reward_i$ is symmetric for any permutation of $i \in \nint$, the value is given by\footnote{Refer \ifodd\full Section \ref{sec:proofs} \else the supplement material \fi for the proofs.},
\begin{flalign}
    \hat{J} = \sup_{\vect{w} \in \mathcal{W}} \int n \Reward_1 \dd  \act^n \dd \model^n (s | \vect{h}) \dd  \mathcal{P}.
\end{flalign}\label{prp:truthfulness}
\end{prp}
If $ \Gn $ is non-truthful, global optimally generally does not hold. 

\label{sec:truthfulness}
\if\full
\begin{table} [t]
\caption{State-action value of $ \Com $ $ Q_i(s_i, \langle z_i, a_i^* \rangle) $}
\centering
        {\small
\begin{tabular}{cccccc}
\hline
&& & \multicolumn{3}{c}{$ z_2 $} \\
&& & True & {\bf False} & Unobserved \\
&& $ (Q_1, Q_2) $ & $ h_2 $ & $ 1-h_2 $ & $ \circ $ \\\hline
& T & $ h_1 $ & $ (c, c) $ & $ (c, c) $ & $(c, c) $ \\
$ z_1 $ & F & $ 1-h_1 $ & $ (c, c) $ & $ (c, c) $ & $ (1, -1) $ \\
& U & $\circ$  & $ (c, c) $ & $ (-1, 1) $ & $ (c/4, c/4) $ \\\hline
\end{tabular}
        }
\label{tbl:expect}
\end{table}

\begin{exam}
Table \ref{tbl:expect} lists the state-action values for the message at $\act \in \mathcal{W}^*(\Com)$.
The best response of messages $ z_i^*:= \mathrm{argmax}_{z_i} Q_i (s, \langle z_i, a_i^* \rangle) $ depends on $ c $ .
    \begin{flalign}
        Q_2(s, \langle h_2, a_2^* \rangle ) - Q_2(s, \langle 1-h_2, a_2^* \rangle ) 
        =& \left( Q_2^* |_{\vect{z} = \langle \circ, 1\rangle} -  Q_2^* |_{\vect{z} = \langle \circ, 0 \rangle} \right) \mathcal{P}^2(\langle \circ, 1\rangle|1) \notag \\
        =& (c - 1 ) (1-\lambda) \lambda. \notag
    \end{flalign}
        Hence, if  $c \ge 1$, $\Com$ is (strongly) truthful.  The strong truthfulness holds for $c > 1$. 
\end{exam}
\fi



\begin{figure}[t]
 \begin{minipage}{0.29\hsize}
 \begin{center}
  \includegraphics[width=0.99\hsize]{img/game-pomdp-ex.png}
 \end{center}
 \end{minipage}
 \begin{minipage}{0.29\hsize}
  \begin{center}
   \includegraphics[width=0.99\hsize]{img/game-pomdp.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.4\hsize}
 \begin{center}
     \small{
\begin{tabular}{ccccc}
\hline
&                       &              & \multicolumn{2}{c}{$a_2$} \\
&                       &  & True          & False           \\
&                       & $(r_1, r_2)$ & $s$          & $1-s$           \\ \hline
\multirow{2}{*}{$a_1$} & T & $s$            & $(c, c)$    & $(1, -1)$   \\
                       & F & $1-s$          & $(-1, 1)$   & $(0, 0)$    \\ \hline
\end{tabular}
    }
 \end{center}
 \end{minipage}
    \caption{
		{\bf Left:} An example of the non-cooperative solutions: $s=1$, $\vect{x} = \langle \circ, 1\rangle$, $\vect{z} = \langle \circ, 0 \rangle $, $\vect{a} = \langle 0, 1 \rangle$, $\vect{r} = \langle -1, 1 \rangle$ and $r_1 + r_2=0 < 2c$.
		{\bf Middle:} One-bit two-way communication game $\Com$.
		{\bf Right:} Reward function $ \mathcal{R}^2 (s, \vect{a}) $. $ c> 0 $ is a constant that determines the nature of the game.
    } 
 \label{fig:com}
\end{figure}

\begin{thm}
    If $ \Gn \in \GameSpace$ is non-truthful, self-play does not converge to the global optimum $ \hat{J} (\Gn) $.
\end{thm}
{\em Proof.} 
Consider an example with two agents and one-bit state $\Com$ as illustrated in Fig. \ref{fig:com}.
$ \State = \Action = \{0, 1 \}, \Obs = \State \cup \{\mathsf{\circ} \} $, and $ p(s) = 1/2 $. 
Agents are given correct information from the environment with a probability of $ \lambda> 0 $:
$ \mathcal{P}(s | s) = \lambda, \, \mathcal{P}(\circ | s) = 1-\lambda $. 
$ q_i(s | x_i, z_j) $ follows a Bernoulli distribution. 
Let $h_i = x_i$.
The agent should infer $p(s)$ from observations and messages $ z_j \in \Message = \Obs $. 

As we can see from the example in Fig. \ref{fig:com} Right, the selfish agent deceives the other agents to maximize their reward.
In the situation, the social welfare $J$ cannot be maximized.
More formally, from Lemma \ifodd\full\ref{lemma:prob-com}\else A.2\fi, if $ c < 1 $, $ J^* (\Com) <\hat{J} (\Com) $ holds. Hence, 
$ \Gn = \Com$ is the counterexample that global optimally does not occur. $ \square $

% ================================================= ====================================
%Without appropriate incentives, the agents will not share the appropriate information they received. 
%The problem is also known as the {\em moral hazard} in the field of economics.
%More formally, we denote the situation as a social dilemma: each agent maximizes the individual value function $ V_i $ without supervision but generally does not maximize the social welfare.

%Before show the example, we show a quite an interesting connection between mechanism design and reinforcement learning.
%In this paper, we assume a utilitarian mechanism designer who wants to maximize the total expected utility of the population. 
%That justifies bringing mechanism design to self-play.
%Let us suppose that $n \ge 2$, and the Nash equilibrium of $ \Reward $ maximizes the sum in full observability.
%These assumptions for the reward are possibly relaxed, but it is not the scope of this paper.
%If all the agents at the equilibrium report the true signal, i.e.,  a certain $ \vect{w}^* \in \mathcal{W}^* (\Gn) $ satisfies $ z_i = h_i,^\forall i \in \nint $ with probability 1, then $ \Gn $ is {\em truthful} \citep{vickrey1961counterspeculation} (or incentive-compatible). 
%In particular, when {\em all} $\vect{w}^* \in \mathcal{W}^*(\Gn)$ satisfies  $ z_i = h_i,^\forall i \in \nint $ with probability 1, $ \Gn $ is {\em strongly truthful} \citep{vickrey1961counterspeculation}.
%Truthfulness and global optimally of self-play is strongly related. %In particular, the following proposition holds.

%The result is quite intuitive. As long as the agents share the correct signal, self-play converges to the global optimum.
%Note that truthfulness is a satisfactory condition.

